Regret Minimization in Partially Observable Linear Quadratic Control

We study the problem of regret minimization in partially observable linear quadratic control systems when the model dynamics are unknown a priori. We propose ExpCommit, an explore-then-commit algorithm that learns the model Markov parameters and then follows the principle of optimism in the face of uncertainty to design a controller. We propose a novel way to decompose the regret and provide an end-to-end sublinear regret upper bound for partially observable linear quadratic control. Finally, we provide stability guarantees and establish a regret upper bound of $\tilde{\mathcal{O}}(T^{2/3})$ for ExpCommit, where $T$ is the time horizon of the problem.

==> macros.tex <==
\newcommand{\alg}{\textsc{\small{GTRPO}}\xspace}
\newcommand{\LQG}{\textsc{\small{LQG}}\xspace}
\newcommand{\POMDP}{\textsc{\small{POMDP}}\xspace}
\newcommand{\MDP}{\textsc{\small{MDP}}\xspace}
\newcommand{\trpo}{\textsc{\small{TRPO}}\xspace}
\newcommand{\ppo}{\textsc{\small{PPO}}\xspace}
\newcommand{\PPO}{\textsc{\small{PPO}}\xspace}
\newcommand*{\Scale}[2][4]{\scalebox{#1}{$#2$}}
\newcommand{\vecy}{\vec y}
\newcommand{\history}{\mathfrak{H}}
\newcommand{\trans}{T}
\newcommand{\obs}{O}
\newcommand{\Texp}{T_{exp}}
\newcommand{\Dexp}{\mathcal{D}_{exp}}

\DeclareMathOperator{\Tr}{Tr}
\newcommand{\ta}{\tilde{A}}
\newcommand{\tb}{\tilde{B}}
\newcommand{\tc}{\tilde{C}}
\newcommand{\tp}{\tilde{P}}
\newcommand{\tl}{\tilde{L}}
\newcommand{\tk}{\tilde{K}}
\newcommand{\tth}{\tilde{\Theta}}

\newcommand{\policy}{\Pi}
\newcommand{\vpi}{{\pi}}
\newcommand{\vobs}{\vec{o}}
\newcommand{\stait}{\omega}
\newcommand{\rxa}{\Gamma}
\newcommand{\rya}{\Upsilon}
\newcommand{\U}{\mathcal{U}}
\newcommand{\Est}{M_1}
\newcommand{\End}{M_2}
\newcommand{\Erd}{M_3}
\newcommand{\decompos}{\gamma}
\newcommand{\pertM}{\Delta M_3}
\newcommand{\pertMM}{\Delta \tilde{M_3}}
\newcommand{\samplenum}{m_s}
\newcommand{\reward}{\Psi}
\newcommand{\tuple}{\mathcal{M}}
\newcommand{\bellman}{\mathcal{E}}
\newcommand{\whole}{\tilde{\mathcal{M}}}
\newcommand{\approxim}{\breve{\mathcal{M}}}
\newcommand{\subst}{{\breve{\eta}}_{\vpi^*}}
\newcommand{\effect}{v}
\newcommand{\belief}{b}
\newcommand{\cost}{c}
\newcommand{\val}{J}
\newcommand{\Qfunc}{Q}

\newcommand{\block}{\Xi}
\newcommand{\vect}{Vec}
\newcommand{\rprob}{z}
\newcommand{\past}{n}
\newcommand{\smucrl}{\textsc{\small{SM-UCRL}}\xspace}
\newcommand{\tslive}{\textsc{\small{TS-LIVE}}\xspace}
\newcommand{\olive}{\textsc{\small{OLIVE}}\xspace}
\newcommand{\cdp}{\textsc{{CDP}}\xspace}
\newcommand{\cdps}{\textsc{{CDPs}}\xspace}
\newcommand{\ts}{\textsc{TS}\xspace}
\newcommand{\ofu}{\textsc{OFU}\xspace}
\newcommand{\ucrl}{\textsc{\small{UCRL}}\xspace}
\newcommand{\mdp}{\textsc{\small{MDP}}\xspace}
\newcommand{\pomdp}{\textsc{\small{POMDP}}\xspace}
\newcommand{\Azuma}{\mathcal{J}}
\newcommand{\Dr}{D_{\text{ratio}}}
\newcommand{\Ke}{\mathcal{K}_\epsilon}
\newcommand{\Le}{L_\epsilon}
\newcommand{\w}{W}
\newcommand{\VV}{B}
\newcommand{\vv}{b}
\newcommand{\HH}{S}
\newcommand{\hhh}{s}
\newcommand{\deltaO}{d_O}

\newcommand*{\defeq}{\mathrel{\vcenter{\baselineskip0.5ex \lineskiplimit0pt
                     \hbox{\scriptsize.}\hbox{\scriptsize.}}}%
                     =}

% Misc symbols
\renewcommand{\Re}{\mathbb{R}}
\newcommand{\calP}{\mathcal P}
\newcommand{\F}{\mathcal F}
\newcommand{\Z}{\mathcal Z}
\newcommand{\A}{\mathcal A}
\newcommand{\B}{\mathcal B}
\newcommand{\X}{\mathcal X}
\newcommand{\T}{\mathcal T}
\newcommand{\KL}{\mathcal D_{KL}}
\newcommand{\wKL}{\wh{\mathcal{D}}_{KL}}
\newcommand{\D}{\mathcal D}
\newcommand{\Gr}{\nabla_{\theta}}
\newcommand{\Greta}{\nabla \eta}
\newcommand{\Grrho}{\nabla \rho}
\newcommand{\Grphi}{\nabla_\phi}
\newcommand{\adv}{A}
\newcommand{\TN}{N}
\newcommand{\hh}{\hat h}
\newcommand{\hL}{\hat L}
\renewcommand{\L}{\mathcal L}
\newcommand{\Hyp}{\mathcal H}
\newcommand{\Y}{\mathcal Y}
\newcommand{\V}{\mathcal V}
\newcommand{\M}{\mathcal M}
\renewcommand{\S}{\mathcal S}
\newcommand{\C}{\mathcal C}
\newcommand{\K}{\mathcal K}
\newcommand{\E}{\mathbb E}
\newcommand{\calE}{\mathcal E}
\newcommand{\Cov}{\textnormal{Cov}}
%\newcommand{\V}{\mathbb V}
\newcommand{\Prob}{\mathbb P}
\newcommand{\I}{\mathbbm 1}
\newcommand{\N}{\mathcal N}
\newcommand{\balpha}{\boldsymbol \alpha}
\newcommand{\bmu}{\boldsymbol \mu}
\newcommand{\bSigma}{\boldsymbol \Sigma}
\newcommand{\bT}{\boldsymbol{T}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\MV}{\textnormal{MV}}
\newcommand{\hMV}{\widehat{\textnormal{MV}}}
\newcommand{\barmu}{\bar\mu}
\newcommand{\hmu}{\hat\mu}
\newcommand{\tmu}{\tilde\mu}
\newcommand{\barvar}{\bar\sigma^2}
%\newcommand{\hvar}{\hat\sigma^2}
\newcommand{\tvar}{\tilde\sigma^2}
\newcommand{\R}{\mathbb{R}}
\newcommand{\hR}{\widehat{\mathcal{R}}}
\newcommand{\tR}{\widetilde{\mathcal R}}
\newcommand{\Cb}{{\mtx{C}}}
%\newcommand{\var}{\sigma^2}
\newcommand{\invdelta}{1/\delta}
\newcommand{\boldR}{\mathbb R}
\newcommand{\eps}{\varepsilon}
\newcommand{\mvlcb}{\textnormal{\texttt{MV-LCB }}}
\newcommand{\ucb}{\textnormal{\textsl{UCB }}}
\newcommand{\ucbv}{\textnormal{\textsl{UCB-V }}}
\newcommand{\mvlcbt}{\textnormal{\texttt{MV-LCB(t) }}}
\newcommand{\htheta}{\hat{\theta}}
\newcommand{\hi}{\hat{i}}
\newcommand{\btheta}{\bar{\theta}}
\newcommand{\tTheta}{\widetilde{\Theta}}



\newcommand{\cvar}{\textnormal{C}}
\newcommand{\hcvar}{\widehat{\textnormal{C}}}
\newcommand{\var}{\textnormal{V}}
\newcommand{\hvar}{\widehat{\textnormal{V}}}
\newcommand{\Pinit}{P_\varnothing}



\newcommand{\avg}[2]{\frac{1}{#2} \sum_{#1=1}^{#2}}
\newcommand{\hDelta}{\widehat{\Delta}}
\newcommand{\hGamma}{\widehat{\Gamma}}

\newcommand{\wt}{\widetilde}
\newcommand{\wh}{\widehat}
\newcommand{\wb}{\overline}
 \newcommand{\mbb}{\mathbbm}

% Propositions
%
%\newtheoremstyle{dotless}{}{}{\itshape}{}{\bfseries}{}{ }{}
%\theoremstyle{dotless}
% \newtheorem{lemma}{Lemma}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{theorem*}{Theorem}[section]
% \newtheorem{corollary}{Corollary}[section]
% \newtheorem{proposition}{Proposition}[section]
% \newtheorem{definition}{Definition}[section]
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{remark}{Remark}[section]
% \newtheorem{proof}{Proof}
% \newtheorem*{proof*}{Proof}

% Misc
%\newcommand{\note}[1]{\textbf{Note.} \textit{#1}}
%\newcommand{\TODO}[1]{(\textbf{TODO: {#1}})}
%\renewcommand{\remark}[1]{\textbf{Remark #1.}}


